Design of a test rig for the investigation of falling film flows with counter-current gas flows

Geothermal phase change probes operate on the principle of falling film evaporation, enabling the efficient use of geothermal heat for space heating applications. Despite successful applications in research, their commercial use is limited. One of the primary reasons for this is the absence of validated models capable of accurately representing the falling film flow coupled with counter-current gas flow within these probes. For this reason, a test rig has been developed to facilitate the validation of future models. This test rig allows for the replication of flow phenomena appearing within geothermal probes under controlled conditions. The test rig was successfully tested within the first measurement campaign presented in this paper. Within the framework of this measurement campaign water was used as liquid due to its similar Kapitza number compared to \(CO_{2}\), typically used within geothermal probes, and humid air as gas. For the gas phase, velocity profiles were measured and for the liquid phase high temporal resolution film thickness measurements were conducted. Both measurement systems show qualitative comparable results to literature. Additionally, the sampled film thickness data were averaged to enable a time-independent interpretation. The investigation of the average film thickness in flow direction, without gas flow, revealed an increase in film thickness along flow direction for \(Re_{film}=500\). In contrast, for \(Re_{film}\geq 980\), an opposing trend was observed. Furthermore, the influence of gas flow on the average film thickness was investigated. The measurement results and high-speed camera images indicate that the test rig is capable of reaching flooding conditions.

==> mwi_bibliography_reserve.tex <==

% Overview of falling film flows (here numerics in horizontal tubes)
@article{ZHAO2022117869,
title = {A comprehensive review on computational studies of falling film hydrodynamics and heat transfer on the horizontal tube and tube bundle},
journal = {Applied Thermal Engineering},
volume = {202},
pages = {117869},
year = {2022},
issn = {1359-4311},
doi = {https://doi.org/10.1016/j.applthermaleng.2021.117869},
url = {https://www.sciencedirect.com/science/article/pii/S135943112101293X},
author = {Chuang-Yao Zhao and Di Qi and Wen-Tao Ji and Pu-Hang Jin and Wen-Quan Tao},
keywords = {Falling film evaporation, Spray evaporation, Refrigeration, Computational fluid dynamics, Film thickness, Heat transfer},
abstract = {Falling film evaporation is a promising technology widely applied in refrigeration, desalination and beyond applications owing to the great advantages. However, the liquid film hydrodynamics and heat transfer performance are studied insufficiently. Compered with experiments, numerical simulations are economical and efficient especially in the study of liquid film, through which some microscopic understandings are expected to be extracted. In this paper, a comprehensive review for a large pool of computational studies about falling liquid film flow and heat transfer on the horizontal tube and tube bundle is presented. Computational methods of liquid gas two-phase flow and mass transfer model, as well as relevant researches were first introduced. Then, the studies on the falling film hydrodynamics, film thickness, sensible heat transfer, flow pattern, evaporation and boiling outside the single tube, tube bundle, special-shaped tube and entire evaporator studied with 2D and 3D models are respectively reviewed in order. Then, the investigations on the falling film breakout and dryout are reviewed. And then, the numerical predictions of falling film thickness and heat transfer coefficient are involved. Afterthat, the benchmark data for falling film numerical simulation are summarized. Finally, some future needs and recommendation relating to crucial technologies that must be solved are proposed.}
}

% desalination citation
@article{MACIVER2005221,
title = {New trend in desalination for Japanese nuclear power plants, based on multiple effect distillation, with vertical titanium plate falling film heat transfer configuration},
journal = {Desalination},
volume = {182},
number = {1},
pages = {221-228},
year = {2005},
note = {Desalination and the Environment},
issn = {0011-9164},
doi = {https://doi.org/10.1016/j.desal.2005.04.014},
url = {https://www.sciencedirect.com/science/article/pii/S0011916405004352},
author = {A. Maciver and S. Hinge and B.J. Andersen and J.B. Nielsen},
keywords = {Desalination, MED, Nuclear power plants, Japan, Alfa laval, Falling film plates},
abstract = {In the last two decades there has been a small but steady replacement of ageing MSF type desalination units installed at Japanese power plants with either MED or RO desalination plants. These have proven to be very competitive and reliable technologies, and the operating experience especially with MED type plants has been very encouraging. The use of desalinated water for Japanese power plants gives the customer significant advantages especially in a land as environmentally conscious as Japan. It is anticipated that the replacement market will continue at the current level and that additional new power plant projects will give increasing consideration to the use of desalination technologies to meet their needs for high quality, and reliable availability, water requirements.}
}

%overview about destillation
@article{BATTISTI2020107873,
title = {A background review on falling film distillation in wetted-wall columns: From fundamentals towards intensified technologies},
journal = {Chemical Engineering and Processing - Process Intensification},
volume = {150},
pages = {107873},
year = {2020},
issn = {0255-2701},
doi = {https://doi.org/10.1016/j.cep.2020.107873},
url = {https://www.sciencedirect.com/science/article/pii/S0255270120300283},
author = {Rodrigo Battisti and Ricardo A.F. Machado and Cintia Marangoni},
keywords = {Falling film distillation, Wetted-Wall columns, Separation efficiency parameters, Constructive column configurations},
abstract = {In response to the worldwide need for more sustainable chemical processes, distillation became target of major efforts for efficiency improvement. Leveraged by process intensification, several technologies have been proposed to reach a more compact, safer, and less energy-intensive equipment. Falling film columns were intensively used for heat and mass transfer research in last century. Noteworthy, studies proposing the falling film technology in distillation condition highlighted numerous advantages, such as low residence time and simple constructive structure when compared to conventional distillation, as well as high transfer rates due to the small thickness that flows in longitudinal direction of the distillation wall. Therefore, this review brings a historical perspective of theoretical and experimental works as well as deposited patents on falling film distillation from the beginning of 20th Century to present. Theoretical background and conceptual aspects related to efficiency improvement and process intensification were deeply discussed, aiming to guideline future perspectives in chemical separations.}
}

@article{NA2020101810,
	
	author = {W. Na and J.W. Zeng and D.Y. Li and Y. Wu and J.S Wu},
	doi = {10.1016/j.scs.2019.101810},
	issn = {2210-6707},
	journal = {Sustainable Cities and Society},
	keywords = {Heat extraction, Horizontal elliptical tube, Film thickness distribution, Spray heat exchanger, Sewage heat pump system},
	pages = {101810},
	title = {Experimental and theory investigations on falling film flow characteristics and heat extraction performance of spray heat exchanger for sewage heat pump system},
	url = {https://www.sciencedirect.com/science/article/pii/S2210670719309333},
	volume = {52},
	year = {2020}
}


@article{NARVAEZROMO20171079,
title = {A critical review of heat and mass transfer correlations for LiBr-H2O and NH3-H2O absorption refrigeration machines using falling liquid film technology},
journal = {Applied Thermal Engineering},
volume = {123},
pages = {1079-1095},
year = {2017},
issn = {1359-4311},
doi = {https://doi.org/10.1016/j.applthermaleng.2017.05.092},
url = {https://www.sciencedirect.com/science/article/pii/S135943111730861X},
author = {Beethoven Narvez-Romo and Marx Chhay and El W. Zavaleta-Aguilar and Jose R. Simoes-Moreira},
keywords = {Falling film, Absorption, Review, Ammonia-water, Lithium bromide-water},
abstract = {This paper presents an extensive review of heat and mass transfer correlations in the framework of sorption machines operating based on the falling film technology, in which ammonia-water and lithium bromide-water are used as the working fluid pairs. Heat and mass transfer correlations are summarized as well as the application range and geometrical configuration. In order to compare the correlations found in the recent and classical literature, typical operation conditions for absorption refrigeration cycles have been adopted. Heat and mass transfer correlations have been evaluated for both working fluid pairs, mapping the possible heat and mass transfer values for refrigeration and air-conditioning applications. The study allowed comparing the two technologies using the same operational conditions. The ascertainment that the transfer correlations may behave differently has been showed. Finally, this work suggests that future researches about heat and mass transfer behavior should be to carry out for realistic operational condition of the absorption refrigeration cycles.}
}

@article{RUI2018450,
title = {Modelling ground source heat pump system by an integrated simulation programme},
journal = {Applied Thermal Engineering},
volume = {134},
pages = {450-459},
year = {2018},
issn = {1359-4311},
doi = {https://doi.org/10.1016/j.applthermaleng.2018.01.123},
url = {https://www.sciencedirect.com/science/article/pii/S1359431117320446},
author = {Yi Rui and Denis Garber and Mei Yin},
keywords = {Ground source heat pump, Finite element, Thermal pile},
abstract = {Ground Source Heat Pump (GSHP) is a technology which can be utilized to offer low carbon emissions heating/cooling and hot water supply. However, improperly designed GSHPs can increase operational costs and often do not provide the expected reduction in emissions. Under the current design approach in the industry, each of the GSHP system components is designed separately. To optimize the trade-offs between the different system components and to account for the uncertainty in thermal behaviour of ground and ground heat exchanger (GHE), we need an integrated approach that can model the system as a whole. In this paper, an integrated model of GSHP systems is developed and tested through a case study of an existing GSHP system in UK. In this integrated model, the GHE is simulated by a computational intensive finite element model, which can quantitatively predict the changes of temperature in the ground heat exchanger and surrounding soil. The close match between the modelled results and the actual data demonstrates the ability of the integrated model to simulate thermal-pile systems with a reasonable level of accuracy.}
}

@article{BLOOMQUIST2003513,
	abstract = {The use of geothermal resources for space heating dominates the direct use industry, with approximately 37\% of all direct use development. Of this, 75\% is provided by district heating systems. In fact, the earliest known commercial use of geothermal energy was in Chaudes-Aigues Cantal, France, where a district heating system was built in the 14th century. Today, geothermal district space heating projects can be found in 12 countries and provide some 44,772 TJ of energy yearly. Although temperatures in excess of 50 °C are generally required, resources as low as 40 °C can be used in certain circumstances, and, if geothermal heat pumps are included, space heating can be a viable alternative to other forms of heating at temperatures well below 10 °C.},
	author = {R.Gordon Bloomquist},
	doi = {10.1016/j.geothermics.2003.06.001},
	issn = {0375-6505},
	journal = {Geothermics},
	keywords = {Direct uses, Space heating, District heating, Absorption technology},
	note = {Selected Papers from the European Geothermal Conference 2003},
	number = {4},
	pages = {513–526},
	title = {Geothermal space heating},
	url = {https://www.sciencedirect.com/science/article/pii/S0375650503000841},
	volume = {32},
	year = {2003}
}

@article{Hagedorn_2024,
	abstract = {This paper examines a 368 m deep geothermal probe for heating an existing building. The geothermal probe based on the thermosyphon principle works with CO2. The working fluid evaporates and condenses in the probe so that no pump is required for transportation. The geothermal probe has an output of up to 22 kW at an underground temperature of up to 18°C. The demand-controlled use of the geothermal probe was investigated and the installed heat pump was optimized for its use. The average COP of the last heating season was between 2,3 and 4,6. For the second heating season the temperature of the soil around the probe is also measured via a distributed temperature sensing system, that covers the whole depth of the probe. It has been shown that the ground temperature only cools down to a certain point and does not fall below this point after a short regeneration period. It was shown that the heat pump with geothermal probe operates at constant temperatures at the evaporator compared to air heat pumps, even at cold outside temperatures.},
	author = {Janina Hagedorn and Robin Kahlfeld and Malte Nageler and Stephan Kabelac},
	doi = {10.1088/1742-6596/2766/1/012106},
	journal = {Journal of Physics: Conference Series},
	month = {may},
	number = {1},
	pages = {012106},
	publisher = {IOP Publishing},
	title = {Investigation of the operating characteristic of a demand-controlled 368 m deep CO2 thermosyphon geothermal borehole heat exchanger for building heating},
	url = {https://dx.doi.org/10.1088/1742-6596/2766/1/012106},
	volume = {2766},
	year = {2024}
}


@article{Ebeling2017,
	abstract = {Geothermal heat pipes are an effective heat source for heat pumps used for space heating. Because the area for the installation of borehole heat exchangers is limited in urban areas (one site per borehole), the maximum heat extractable from one borehole shall rise. In cooperation with the FKW Hannover, the Institute for Thermodynamics of the Leibniz University of Hannover is investigating the thermodynamic behavior of CO2 driven geothermal heat pipes of higher thermal power. Therefore two different types of geothermal heat pipes with a length of 400m each have been installed. Furthermore a numerical simulation of the heat and mass transfer within the pipes is under development. The experimental setup and first results of the experiments are presented as well as the current status of the numerical simulation. A comparison of the two different types of heat pipes and a comparison of the experimental data with the numerical simulation is given.},
	author = {JC.Ebeling, S.Kabelac, S.Luckmann and H.Kruse},
	doi = {10.1007/s00231-017-2014-7},
	journal = {Heat Mass Transfer},
	pages = {3257–3265},
	publisher = {},
	title = {Simulation and experimental validation of a 400 m vertical CO2 heat pipe for geothermal application},
	url = {https://doi.org/10.1007/s00231-017-2014-7},
	volume = {53},
	year = {2017}
}

@article{Kruse2010,
	abstract = {},
	author = {H.Kruse and H.Russmann},
	doi = {},
	journal = {International High Performance Buildings Conference.},
	pages = {},
	publisher = {},
	title = {The Status of Development and Research on CO2 Earth Heat Pipes for Geothermal Heat Pumps},
	url = {http://docs.lib.purdue.edu/ihpbc/51},
	volume = {Paper 51.},
	year = {2010}
}

@inbook{Storch2018,
	abstract = "Für die Nutzung der Oberflächennahen Geothermie als erneuerbare Energiequelle zur Bereitstellung von Heizwärme im Gebäudebereich existiert eine Vielzahl an unterschiedlichen Wärmeentzugssystemen. Bei allen Systemen sind die thermophysikalischen als auch die materialspezifischen Parameter (Wärmeleitfähigkeit, spezifische Wärmekapazität, Dichte etc.) u. a. des Erdreiches, des Bohrlochs, des Zementes und der Geothermiesonde oder des Kollektors wichtige Einflussgrößen und müssen in der Planung und Auslegung entsprechend berücksichtigt werden. Ein innovatives und zugleich sehr effizientes Prinzip für den Wärmeentzug aus dem Erdreich stellt eine Anwendung der Fallfilmverdampfung in einem geothermischen Thermosiphon (auch Phasenwechselsonde genannt) in Kombination mit einer Wärmepumpe dar. Erste Anwendungen von Thermosiphons in oberflächennahen Erdschichten datieren aus der Zeit um 1960, z. B. in Alaska, wobei es sich vorwiegend um die Untergrundstabilisierung in Regionen mit Permafrostböden handelte. Das wohl bekannteste Projekt ist die 1977 fertiggestellte Trans-Alaska-Pipeline, welche auf ca. 730 km mit über 122.000 Thermosiphons stabilisiert wird. Seit 1997 wird dieses einfache Prinzip auch in Kombination mit Wärmepumpen zur Wärmeversorgung von Gebäuden genutzt. In diesem Beitrag werden hierzu die Funktionsweise und die Betriebsbedingungen von geothermischen Phasenwechselsonden mit den Vor- und Nachteilen gegenüber Flüssigkeitszirkulationssonden auf dem neuesten Stand der Forschung sowohl für Anwender als auch für Wissenschaftler umfangreich dargelegt. Dabei werden die ablaufenden Prozesse für verschiedene Betriebsphasen (Start, zyklischer oder dauerhafter Wärmeentzug, Regeneration) u. a. hinsichtlich der Filmausbreitung, der Poolaktivität und einer energetischen Bewertung beschrieben. Abschließend werden kurz zukünftige Forschungsfelder geothermischer Phasenwechselsonden umrissen sowie relevante Perspektiven und Herausforderungen diskutiert.",
	address = "Berlin, Heidelberg",
	author = "Storch, Thomas and Grab, Thomas and Groß, Ulrich",
	booktitle = "Handbuch Oberflächennahe Geothermie",
	doi = "10.1007/978-3-662-50307-2_13",
	editor = "Bauer, Mathias and Freeden, Willi and Jacobi, Hans and Neu, Thomas",
	isbn = "978-3-662-50307-2",
	pages = "409–449",
	publisher = "Springer Berlin Heidelberg",
	title = "Geothermische Phasenwechselsonden als Wärmeentzugssystem",
	url = "https://doi.org/10.1007/978-3-662-50307-2_13",
	year = "2018"
}

@book{StorchDiss,
    author ="T.Storch",
    title ="Grundlegende Untersuchungen zum Wirkprinzip von geothermischen Phasenwechselsonden. Dissertation." ,
    publisher ="Sierke Verlag, Freiberg," ,
    ISBN = "978-3-86844-707-1",
    year = "2015",
    url = "http://doi.org/10.14626/9783868447088", 
}

@article{KOFMAN201722,
	abstract = {We report an experimental investigation of a falling water film sheared by a turbulent counter-current air flow in an inclined rectangular channel. Film thickness and wave velocity measurements associated with visual observation are conducted to study the influence of the air flow on controlled traveling waves consisting of a large wave hump preceded by capillary ripples. First, we focus on the variation of the shape, amplitude and velocity of the waves as the gas velocity is gradually increased. We demonstrate that the amplitude of the main hump grows substantially even for moderate gas velocities, whereas modification of the wave celerity becomes significant above a specific gas velocity around 4 m/s, associated with an alteration of the capillary region. The influence of the gas flow on 3D secondary instabilities of the solitary waves detected in a previous study Kofman et al. (2014), namely rugged or scallop waves, is also investigated. We show that the capillary mode is damped while the inertial mode is enhanced by the interfacial shear. Next, the gas velocity is increased until the onset of upstream-moving patterns referred to as flooding in our experiments. At moderate inclination angles (typically < 7 ○), flooding occurs for a gas velocity around 8 m/s and is initiated at the scallop wave crests by a backward wave-breaking phenomenon preceded by the onset of ripples on the flat residual film separating two waves. At high inclination angle, a rapid development of solitons is observed as the air velocity is increased preventing the waves to turn back. Finally, at high liquid Reynolds number, sudden and intermittent events are triggered consisting of very large amplitude waves that go back upwards very fast. These “slugs” either extend over the whole width of the channel or are very localized and can thus potentially evolve towards atomization.},
	author = {N. Kofman and S. Mergui},
	doi = {10.1016/j.ijmultiphaseflow.2017.05.007},
	issn = {0301-9322},
	journal = {International Journal of Multiphase Flow},
	keywords = {Falling liquid films, Counter-current gas flow, Solitary waves, Flooding},
	pages = {22–34},
	title = {Characteristics of solitary waves on a falling liquid film sheared by a turbulent counter-current gas flow},
	url = {https://www.sciencedirect.com/science/article/pii/S0301932216306978},
	volume = {95},
	year = {2017}
}

@article{HUANG2014125,
	abstract = {Water–air countercurrent flow in a rectangular channel is studied experimentally in this study. The experiment is carried out in a large scale facility that consists of a large scale flow channel and a rotatable operating platform which provides different inclination conditions. This paper focuses on the study of film behavior, such as film thickness and surface wave, in countercurrent flow. Optical thickness probe, hot wire anemometry and high speed camera are applied to perform the data measurement. The results show that the film thickness variation in the large scale channel under countercurrent flow condition is different from the results from small scale tests. The critical air velocity, which is usually considered as the proof of flooding onset, is discussed for different film Reynolds numbers. Moreover, the droplet entrainment plays an important role under high speed air flow conditions. The observation of the surface wave is also conducted to supplement the analysis of film surface variation.},
	author = {X.G. Huang and Y.H. Yang and P. Hu and K. Bao},
	doi = {10.1016/j.anucene.2014.02.005},
	issn = {0306-4549},
	journal = {Annals of Nuclear Energy},
	keywords = {Countercurrent, Onset of flooding, Film thickness, Surface wave, Large scale test, PCCS},
	pages = {125–133},
	title = {Experimental study of water–air countercurrent flow characteristics in large scale rectangular channel},
	url = {https://www.sciencedirect.com/science/article/pii/S0306454914000759},
	volume = {69},
	year = {2014}
}


@phdthesis{tuprints8742,
        language = {de},
          school = {Technische Universit{\"a}t Darmstadt},
         address = {Darmstadt},
            year = {2019},
          author = {Timm Schr{\"o}der},
           title = {Str{\"o}mungscharakteristika und W{\"a}rme{\"u}bertragung eines angeregten Fallfilms},
             url = {http://tuprints.ulb.tu-darmstadt.de/8742/},
        abstract = {Fallfilme werden in vielen technischen Prozessen zur K{\"u}hlung, Kondensation und Verdampfung verwendet. Die Hydrodynamik und die W{\"a}rme{\"u}bertragung dieser welligen Fl{\"u}ssigkeitsfilme sind von Bedeutung zur Auslegung entsprechender Anlagen. In der Literatur wird die Hydrodynamik von d{\"u}nnen Filmen an senkrechten W{\"a}nden ausf{\"u}hrlich beschrieben. Dort wurde gezeigt, dass die Wellen des Films einen positiven Einfluss auf die W{\"a}rme{\"u}bertragung haben. Ausf{\"u}hrliche Untersuchungen zum Einfluss der Anregungsfrequenz der Wellen sowie deren Amplitude auf den W{\"a}rmetransport des Films wurden jedoch bisher nicht hinreichend durchgef{\"u}hrt.  Aus diesem Grund wurde in der vorliegenden Arbeit gezielt der Einfluss der Wellenanregung auf die W{\"a}rme{\"u}bertragung untersucht. So soll f{\"u}r dieses Themengebiet eine fundierte Grundlage f{\"u}r folgende Arbeiten geschaffen werden. Daf{\"u}r wurde ein Versuchsstand aufgebaut, mit dem die Str{\"o}mungscharakteristika und die W{\"a}rme{\"u}bertragung eines definiert periodisch angeregten Fallfilms hoch aufgel{\"o}st untersucht werden k{\"o}nnen. Mittels eines chromatisch-konfokalen Abstandsmesssystems wurde die Filmdicke erfasst und mit einem Kamerasystem die Filmoberfl{\"a}che fotografiert und ausgewertet. Die W{\"a}rme{\"u}bertragung wurde mit Wandtemperaturmessungen analysiert.  Die durchgef{\"u}hrten Experimente wurden in einem weiten Parameterbereich mit den gezielt variierten Parametern Anregungsfrequenz sowie -amplitude, Fluidmassenstrom, W{\"a}rmestromdichte und Neigungswinkel der Fallwand durchgef{\"u}hrt. Zun{\"a}chst konnte gezeigt werden, dass sich die Wellenformen abh{\"a}ngig von der Anregungsfrequenz entlang der Str{\"o}mungsrichtung unterschiedlich entwickeln. Weiterhin hat die initiale Amplitude der periodischen Anregung, auf die in bisherigen Arbeiten nicht eingegangen wurde, einen deutlichen Einfluss auf die Entwicklung der Wellen. Zu den weiteren untersuchten Wellencharakteristika z{\"a}hlen die mittlere Filmdicke, die Wellenfrequenz, die Wellenmaxima sowie -minima, die Filmdickenverteilung, die Wellenl{\"a}nge und -geschwindigkeit.  Ein Vergleich der experimentellen Ergebnisse mit extrapolierten bekannten Korrelationen lieferte keine ausreichende {\"U}bereinstimmung und die Parameter der Korrelationen wurden an die experimentellen Daten angepasst. Durch die Analysen der Wandtemperaturmessungen zeigte sich ebenfalls ein starker frequenzabh{\"a}ngiger Einfluss der Wellenanregung auf die W{\"a}rme{\"u}bertragung. In bestimmten Frequenzbereichen konnte der W{\"a}rmetransport verbessert werden. Diese Frequenzbereiche korrespondieren mit dem Auftreten ausgepr{\"a}gter Wellenminima in der Filmstr{\"o}mung.}
}

@article{ZHOU2009273,
	abstract = {An experimental investigation of wavy water film falling down a flat plate has been carried out using confocal chromatic sensoring technique to determine the instantaneous and statistical characteristics of the film. The experiments involved three parameters: liquid feed mode, Reynolds number and plate inclination angle. The present time–average film thickness data is compared with the previous experimental and theoretical results showing a good agreement. A new correlation for the average film thickness is suggested. Our results show that the liquid feed mode has a vital influence on the film thickness and that the film thickness increases with Reynolds number and decreased plate inclination angle. The root–mean–square value of the film thickness fluctuations depends non-monotonically on the film Reynolds number. The corresponding mechanisms are analyzed.},
	author = {D.W. Zhou and T. Gambaryan-Roisman and P. Stephan},
	doi = {10.1016/j.expthermflusci.2008.09.003},
	issn = {0894-1777},
	journal = {Experimental Thermal and Fluid Science},
	keywords = {Falling liquid film, Film thickness, Interfacial waves, Laminar flow},
	number = {2},
	pages = {273–283},
	title = {Measurement of water falling film thickness to flat plate using confocal chromatic sensoring technique},
	url = {https://www.sciencedirect.com/science/article/pii/S0894177708001337},
	volume = {33},
	year = {2009}
}


@article{STUCHELI1976369,
	abstract = {An integral method is used to obtain a closed form expression for the determination of hydrodynamic entrance length for falling liquid films emerging from a flat slit and flowing in laminar flow along an inclined flat plate. The results obtained from the present analysis are compared with the experimental data and numerical solutions and found to be in good agreement with them.},
	author = {A. Stücheli and M.N. Özişik},
	doi = {10.1016/0009-2509(76)80006-1},
	issn = {0009-2509},
	journal = {Chemical Engineering Science},
	number = {5},
	pages = {369–372},
	title = {Hydrodynamic entrance lengths of laminar falling films},
	url = {https://www.sciencedirect.com/science/article/pii/0009250976800061},
	volume = {31},
	year = {1976}
}

@article{DROSOS200651,
	abstract = {Results are reported of an experimental investigation of gas–liquid counter-current flow in a vertical rectangular channel with 10mm gap, at rather short distances from liquid entry. Flooding experiments are carried out using air and various liquids (i.e., water, 1.5\% and 2.5\% aqueous butanol solutions) at liquid Reynolds numbers ReL<350. Visual observations and fast recordings suggest that the onset of flooding at low ReL (<250) is associated with liquid entrainment from isolated waves, whereas “local bridging” is dominant at the higher ReL examined in this study. Significant reduction of flooding velocities is observed with decreasing interfacial tension, as expected. Instantaneous film thickness measurements show that under conditions approaching flooding, a sharp increase of the mean film thickness, of mean wave amplitude and of the corresponding RMS values takes place. Film thickness power spectra provide evidence that by increasing gas flow the wave structure is significantly affected; e.g., the dominant wave frequency is drastically reduced. These data are complemented by similar statistical information from instantaneous wall shear stress measurements made with an electrochemical technique. Power spectra of film thickness and of shear stress display similarities indicative of the strong effect of waves on wall stress; additional evidence of the drastic changes in the liquid flow field near the wall due to the imposed gas flow, even at conditions below flooding, is provided by the RMS values of the wall stress. A simple model is presented for predicting the mean film thickness and mean wall shear stress under counter-current gas–liquid flow, below critical flooding velocities.},
	author = {E.I.P. Drosos and S.V. Paras and A.J. Karabelas},
	doi = {10.1016/j.ijmultiphaseflow.2005.07.005},
	issn = {0301-9322},
	journal = {International Journal of Multiphase Flow},
	keywords = {Counter-current gas–liquid flow, Narrow vertical channel, Flooding, Film characteristics, Wall shear stress},
	number = {1},
	pages = {51–81},
	title = {Counter-current gas–liquid flow in a vertical narrow channel—Liquid film characteristics and flooding phenomena},
	url = {https://www.sciencedirect.com/science/article/pii/S0301932205001102},
	volume = {32},
	year = {2006}
}

@article{SAYEGH2022104170,
title = {Impact of physico-chemical properties on falling liquid films flow over flat and corrugated surfaces},
journal = {International Journal of Multiphase Flow},
volume = {155},
pages = {104170},
year = {2022},
issn = {0301-9322},
doi = {https://doi.org/10.1016/j.ijmultiphaseflow.2022.104170},
url = {https://www.sciencedirect.com/science/article/pii/S0301932222001562},
author = {M. Al Sayegh and D. Rouzineau and M. Meyer and E. Cid and P. Alix and C. Dalmazzone and John Roesler},
keywords = {Thin-film flow, Gas-liquid interface, Physico-chemical properties, Local-scale measurements, Fluorescence imaging method},
abstract = {In this paper, an optical technique based on fluorescence intensity is applied and calibrated to simultaneously measure film thickness (up to 8 mm) and interfacial velocity of the liquid film flow. Thus, thin-film flows at intermediate and low Reynolds number (13 < Re < 290) are experimentally studied with special attention given to the spatial variation, the frequency of the waves, and interfacial liquid velocity associated with global visual observation. Two fluids (water-ethanol mixture) characterized by low surface tension (s = 35 and 50 mN/m) and three fluids (water-glycerin mixture) with high viscosity (� = 5, 10, and 15 mPa.s) are used to investigate the influence of physico-chemical properties on thin-film flow on flat and corrugated plate topologies. First, the effect of physico-chemical properties on the global variation of waves shape and instability evolution has been investigated. Different work fluids were used in the same experimental conditions on a flat plate. Results showed that decreasing surface tension has a stabilizing effect on the flow, dampening the capillary waves that should otherwise arise. At high viscosity, solitary waves with high thickness followed by an undisturbed thin-film with a constant thickness appear. The impact of liquid flow rate and inclination (? = 10� and 20�) was also studied. It shows that at higher inclination the film thickness decreases and then increases as the liquid flow rate increases. Next, the impact of counter-current gas was studied and we demonstrated that the amplitude of the main waves significantly increases even at low gas velocity while the effect on the velocity of the wave starts to be significant at a counter-current gas velocity of 3 � 4 m/s. Finally, the effect of the corrugation of the solid plate at a high inclination angle (? = 60�) shows the onset of the breaking waves phenomenon, especially for fluids with low surface tension.}
}

@phdthesis{Al-Sibai_diss,
        language = {de},
          school = {Rheinisch-Westf{\"a}lischen Technischen Hochschule Aachen},
         address = {Aachen},
            year = {2004},
          author = {F. Al-Sibai},
           title = {Experimentelle Untersuchung der Str{\"o}mungscharakteristik
und des W{\"a}rme{\"u}bergangs bei welligen Rieselfilmen},
             url = {https://publications.rwth-aachen.de/record/59863/files/59863.pdf},
        abstract = {
}
}

@article{Nusselt,
title = {Impact of physico-chemical properties on falling liquid films flow over flat and corrugated surfaces},
journal = {Zeitschrift des Vereines Deutscher Ingenieure},
volume = {60(3)},
pages = {541-546},
year = {2022},
issn = {},
doi = {},
url = {},
author = {W.Nusselt},
keywords = {}
}

@article{Kapitza,
title = {Wave flow of thin layers of a viscous fluid. Collected Papers of P.L.Kapitza,
journal = {Elsevier},
volume = {},
pages = {662-709},
year = {1965},
issn = {},
doi = {https://doi.org/10.1016/B978-0-08-010973-2.50013-6},
url = {},
author = {P.L..Kapitza},
keywords = {}
}
}
